Ghosts of Order on the Frontier of Chaos

What kinds of motion can occur in classical mechanics? We address this question by looking at the structures traced out by trajectories in phase space; the most orderely, completely integrable systems, are charactrized by phase trajectories confined to low-dimensional, invariant tori. The KAM theory examines what happens to the tori when an integrable system is subjected to a small perturbation and finds that, for small enough perturbations, most of them survive. The KAM theory is mute on the suject of the disrupted tori, but, for two dimensional systems, Aubry and Mather discovered an astonishing picture: the broken tori are replaced by "cantori", tattered, Cantor-set remnants of the original invariant curves. We seek to extend Aubry and Mather's picture to higher dimensional systems and report two kinds of studies; both concern perturbations of a completely integrable, four-dimensional symplectic map. In the first study we compute some numerical approximations to Birkhoff periodic orbits; sequences of such orbits should approximate any higher dimensional analogs of the cantori. In the second study we prove converse KAM theorems; that is, we use a combination of analytic arguments and rigorous, machine-assisted computations to find perturbations so large that no KAM tori survive. We are able to show that the last few of our Birkhoff orbits exist in a regime where there are no tori.

==> Abstract.tex <==
\begin{center}
	\\
    {\bf Abstract}\\
\end{center}

What kinds of motion can occur in classical mechanics?
We address this question by looking at the
structures traced out by trajectories in phase space;
the most orderely, completely integrable systems, are charactrized
by phase trajectories confined to low-dimensional, invariant tori.
The KAM theory examines what happens to the tori when an
integrable system is subjected to a small perturbation and finds that,
for small enough perturbations, most of them survive.

The KAM theory is mute on the suject of the disrupted tori, but,
for two dimensional systems, Aubry and Mather discovered an astonishing
picture: the broken tori are replaced by ``cantori'', 
tattered, Cantor-set remnants of the original invariant curves.
We seek to extend Aubry and Mather's picture to higher 
dimensional systems and report two kinds of studies;
both concern perturbations of a completely integrable, 
four-dimensional symplectic map.  In the first study we compute
some numerical approximations to Birkhoff periodic orbits; sequences
of such orbits should approximate any higher dimensional analogs 
of the cantori.  In the second study we prove converse KAM theorems;
that is, we use a combination of analytic arguments and rigorous,
machine-assisted computations to find perturbations so large that
no KAM tori survive.  We are able to show that the last few of our
Birkhoff orbits exist in a regime where there are no tori.


==> appendices/code/apmPrinth.tex <==
\begin{verbatim} 


\end{verbatim}


==> appendices/code/apmSpecialh.tex <==
\begin{verbatim} 
# define MAX_TRIG_TERMS  100
# define DFLT_TRIG_DP    20

# define PI_DP	    (sizeof(pi_str) / sizeof(char) - 3)

# ifndef YES
# define YES  1
# define NO   0
# endif 

# ifndef m_swap
# define m_swap(x,y,t)	(t=x, x=y, y=t) 
# endif 

extern APM    zero, one, two ;
extern APM    pi, two_pi, half_pi, threeHalf_pi, eighths_2pi[8] ;
extern APM    Theta, scratch, xMod2pi, Theta_sq, Answer ;
extern APM    Factrl, coef, apmOrder ;
extern APM    approx[2], diff, ub_diff ;
extern int    trig_dp, specialsInit ;
extern int    trig_terms, dp_lost ;
extern char   pi_str[] ;
\end{verbatim}


==> converse/head3.tex <==
%
%	A few boldface math symbols to represent multidimensional 
%	objects.
%
\newcommand{\id}{{\bf I}}
\newcommand{\bfd}{{\bf d}}
\newcommand{\bfm}{{\bf m}}
\newcommand{\bfp}{{\bf p}}
\newcommand{\bfL}{{\bf L}}
\newcommand{\bfu}{{\mbox{\boldmath $u$}}}
\newcommand{\bfv}{{\mbox{\boldmath $v$}}}
\newcommand{\bfx}{{\mbox{\boldmath $x$}}}
\newcommand{\bpsi}{{\mbox{\boldmath $\psi$}}}
\newcommand{\bbeta}{{\mbox{\boldmath $\beta$}}}
\newcommand{\bthet}{{\mbox{\boldmath $\theta$}}}
\newcommand{\bLam}{{\mbox{\boldmath $\Lambda$}}}
%
%	Some extra mathematical symbols relating to matrices
%
\newcommand{\lamM}[1]{{\lambda_{-}({#1})}}
\newcommand{\lamP}[1]{{\lambda_{+}({#1})}}
\newcommand{\Tr}[1]{{{\rm Tr}\,[{#1}]}}
\newcommand{\TrP}{{\rm Tr}_{max}}
\newcommand{\TrM}{{\rm Tr}_{min}}
\newcommand{\iprod}[2]{{\langle {#1}, {#2} \rangle}}
%
%	Yet more symbols
%
\newcommand{\Veps}{{V_{\epsilon}}}
\newcommand{\Vtrg}{{V_{trig}}}
\newcommand{\bfxStar}{{\bfx^{\star}}}


==> numres/lyap.tex <==
\section{ Lyapunov Exponents}
\label{sec:Lyap}
     In the preceeding section we noted that the shape of the orbit changes
abruptly when the exponents of the orbit depart from the unit circle.  Here we
will discuss what can be said about the exponents and show the numerically
computed exponents for our states.  Since we study periodic orbits the 
Lyapunov exponents are just eigenvalues\thesisfootnote{
	In practice the accurate, direct calculation of the matrix
	product in (\ref{eq:DF}) is not possible.  See  
	Appendix~{\ref{sec:NumMeth}}.
	}
of
\begin{equation}
    \left. DF^q \right|_{(x_0, p_0)} \;\; = \;\;
    \left. DF \right|_{(x_{q-1}, p_{q-1})} \circ  
    \left. DF \right|_{(x_{q-2}, p_{q-2})} \circ \cdots \circ 
    \left. DF \right|_{(x_0, p_0)} 
\label{eq:DF}
\end{equation}
From \ref{eq:map} we can calculate
\begin{displaymath}
%
%
DF_{x_0} \; = \; \left[ 
		    \begin{array}{cc}
			\frac{\displaystyle \partial p'}
			     {\displaystyle \partial x} &
			\frac{\displaystyle \partial p'}
			     {\displaystyle \partial p}  \\
%
			\frac{\displaystyle \partial x'}
			     {\displaystyle \partial x} &
			\frac{\displaystyle \partial x'}
			     {\displaystyle \partial p} 
		    \end{array}
		\right]
	\; = \;
		\left[
		   \begin{array}{cc}
		       -\frac{\displaystyle \partial^2 P_\epsilon}
			     {\displaystyle \partial x^2} &
		       {\bf I}  \\
%
		       {\bf I} + 
		       \frac{\displaystyle \partial^2 P_\epsilon}
			    {\displaystyle \partial x^2} &
		       -{\bf I} 
		    \end{array}
		\right]
\end{displaymath}
where {\bf I} is the {\em d\/}-dimensional identity matrix and
$\partial^2 P_\epsilon / \partial x^2$ is the Hessian of the
perturbation.
Each of the $ \left. DF \right|_{(x_i, p_i)} $ may be written as
a real symplectic matrix and so the entire product is sympectic too.
The eigenvalues of $DF$ may come in reciprocal pairs 
\mbox{ $(\lambda_0, 1/\lambda_0)$ } and 
\mbox{ $(\lambda_1, 1/\lambda_1)$ }.  Initially all four are equal to 
one.  As the perturbation increases first one pair, then the other,
depart from the unit circle.  At about the same parameter value for
which the first pair leaves the circle we see the minimizing state
contract along the filaments.   For large enough perturbation both
pairs are non-zero and the distribution along the direction of the
filaments is also Cantor-like.  See figure~(\ref{fig:Lyaps}).

\begin{figure}
\vspace{2.5in}
	\caption{ \em   The Lyapunov exponents for the rotation 
			vectors \mbox{$(1432,1897)/2513$} (left)
			and \mbox{$(377,2330)/3770$} (right).}
\label{fig:Lyaps}
\end{figure}

